The complex projective plane as a ball quotient

In 1986, Deligne and Mostow constructed a ball quotient $\mathbb{B}^2 / \Gamma$ biholomorphic to the complex projective plane $\mathbb{P}^2$ whose branch locus is a line arrangement. In this paper, we show that if $\mathbb{P}^2$ is realized as a ball quotient whose branch divisor $D$ is an arrangement of smooth pairwise normal-crossing curves, then the orbifold $(\mathbb{P}^2,D)$ is isomorphic to either the Deligne-Mostow example or a certain degree 9 cover of it. This classification of "ball quotient structures" on $\mathbb{P}^2$ generalizes the $\mathbb{P}^1$ case due to Poincar\'e.

==> 029-09-resources/singularity-coefficients.tex <==
a, b & (a,b \geq 2) & \SetCell[c=2]{l} 1 - \frac{ 1 }{ b } - \frac{ 1 }{ a } + \frac{ 1 }{ ab } & 
    & 0 & \\
\hline
2, 2, c & (c \geq 2) & \SetCell[c=2]{l} \frac{ 1 }{ 2 } - \frac{ 1 }{ c } + \frac{ 3 }{ 4c^2 } & 
    & 0 & \\
2, 3, 3 & 
    & \frac{ 43 }{ 144 } & \approx 0.30
    & 0 & \\
2, 3, 4 & 
    & \frac{ 65 }{ 192 } & \approx 0.34
    & 0 & \\
2, 3, 5 & 
    & \frac{ 147 }{ 400 } & \approx 0.37
    & 0 & \\
% \hline
% 2(2)b & (b \geq 2) & \SetCell[c=2]{l} - \frac{ 1 }{ 2 } - \frac{ 1 }{ b } + \frac{ 3 }{ 2b^2 } &  & \SetCell[c=2]{l} - \frac{ 3 }{ 4 } + \frac{ 3 }{ 4b } & \\
% 2(m)2 & (m \geq 2) & \SetCell[c=2]{l} - \frac{ m }{ 2 } + \frac{ 3 }{ 4m } &  & \SetCell[c=2]{l} - \frac{ 3 }{ 4 } + \frac{ 3 }{ 4m } & \\
% 2(3)3 & 
%     & - \frac{ 23 }{ 16 } & \approx -1.44
%     & - \frac{ 3 }{ 4 } & = -0.75\\
% 3(2)3 & 
%     & - \frac{ 53 }{ 72 } & \approx -0.74
%     & - \frac{ 5 }{ 8 } & \approx -0.62\\
% 2(4)3 & 
%     & - \frac{ 103 }{ 48 } & \approx -2.15
%     & - \frac{ 15 }{ 16 } & \approx -0.94\\
% 2(3)4 & 
%     & - \frac{ 95 }{ 64 } & \approx -1.48
%     & - \frac{ 7 }{ 8 } & \approx -0.88\\
% 3(2)4 & 
%     & - \frac{ 71 }{ 96 } & \approx -0.74
%     & - \frac{ 11 }{ 16 } & \approx -0.69\\
% 2(5)3 & 
%     & - \frac{ 679 }{ 240 } & \approx -2.83
%     & - \frac{ 11 }{ 10 } & = -1.1\\
% 2(3)5 & 
%     & - \frac{ 599 }{ 400 } & \approx -1.50
%     & - \frac{ 19 }{ 20 } & = -0.95\\
% 3(2)5 & 
%     & - \frac{ 439 }{ 600 } & \approx -0.73
%     & - \frac{ 29 }{ 40 } & \approx -0.72\\
% \hline
% 2(m)2,c & (m,c \geq 2) & \SetCell[c=2]{l} - \frac{ m }{ 2 } + 1 - \frac{ 1 }{ c } + \frac{ 3 }{ 4c^2m } &  & \SetCell[c=2]{l} - \frac{ 3 }{ 4c } + \frac{ 3 }{ 4cm } & \\
% 2(2)3,2 & 
%     & - \frac{ 47 }{ 96 } & \approx -0.49
%     & - \frac{ 5 }{ 16 } & \approx -0.31\\
% \hline
% 2_{(2,t)} & (t \text{ odd} \geq 3) & \SetCell[c=2]{l} - \frac{ 3 }{ 2 } + \frac{ 3 }{ 2t } &  & \SetCell[c=2]{l} \frac{ 3t }{ 4 } - \frac{ 9 }{ 4 } + \frac{ 3 }{ 2t } & \\
% 3_{(2,3)} & 
%     & - \frac{ 7 }{ 8 } & \approx -0.88
%     & \frac{ 5 }{ 8 } & \approx 0.62\\
% 2_{(3,4)} & 
%     & - \frac{ 23 }{ 16 } & \approx -1.44
%     & \frac{ 43 }{ 16 } & \approx 2.69\\
% 4_{(2,3)} & 
%     & - \frac{ 23 }{ 32 } & \approx -0.72
%     & \frac{ 11 }{ 16 } & \approx 0.69\\
% 2_{(3,5)} & 
%     & - \frac{ 119 }{ 80 } & \approx -1.49
%     & \frac{ 79 }{ 20 } & = 3.95\\
% 3_{(2,5)} & 
%     & - \frac{ 119 }{ 120 } & \approx -0.99
%     & \frac{ 87 }{ 40 } & \approx 2.17\\
% 5_{(2,3)} & 
%     & - \frac{ 119 }{ 200 } & \approx -0.59
%     & \frac{ 29 }{ 40 } & \approx 0.72\\
% \hline
% 2_{(2,t)}, b & (t \text{ odd} \geq 3, b \geq 2) & \SetCell[c=2]{l} - \frac{ 1 }{ 2 } - \frac{ 1 }{ b } + \frac{ 3 }{ 2b^2t } &  & \SetCell[c=2]{l} \frac{ 3t }{ 4 } - \frac{ 3 }{ 2 } - \frac{ 3 }{ 4b } + \frac{ 3 }{ 2bt } & \\
% \hline
% 2_{(2,3)}(3)2 & 
%     & - \frac{ 47 }{ 32 } & \approx -1.47
%     & \frac{ 5 }{ 16 } & \approx 0.31\\


==> 029-09-resources/singularity-pair-coefficients.tex <==
a, \boldsymbol{b} & (a,b \geq 2) & 1 - \frac{ 1 }{ a }\\
\hline
\mathbf{2}, 2, a & (a \geq 2) & \frac{ 1 }{ 2a }\\
\mathbf{2}, 3, 3 &  & \frac{ 1 }{ 12 }\\
\mathbf{2}, 3, 4 &  & \frac{ 1 }{ 24 }\\
\mathbf{2}, 3, 5 &  & \frac{ 1 }{ 60 }\\
\hline
2, 2, \mathbf{3} &  & \frac{ 1 }{ 2 }\\
2, \mathbf{3}, 3 &  & \frac{ 5 }{ 12 }\\
2, \mathbf{3}, 4 &  & \frac{ 3 }{ 8 }\\
2, \mathbf{3}, 5 &  & \frac{ 7 }{ 20 }\\
\hline
2, 2, \mathbf{4} &  & \frac{ 5 }{ 8 }\\
2, 3, \mathbf{4} &  & \frac{ 13 }{ 24 }\\
\hline
2, 2, \mathbf{5} &  & \frac{ 7 }{ 10 }\\
2, 3, \mathbf{5} &  & \frac{ 37 }{ 60 }\\
\hline
2, 2, \boldsymbol{b} & (b \geq 6) & 1 - \frac{ 3 }{ 2b }\\

